Key Design Choices in Source-Free Unsupervised Domain Adaptation: An In-depth Empirical Analysis

This study provides a comprehensive benchmark framework for Source-Free Unsupervised Domain Adaptation (SF-UDA) in image classification, aiming to achieve a rigorous empirical understanding of the complex relationships between multiple key design factors in SF-UDA methods. The study empirically examines a diverse set of SF-UDA techniques, assessing their consistency across datasets, sensitivity to specific hyperparameters, and applicability across different families of backbone architectures. Moreover, it exhaustively evaluates pre-training datasets and strategies, particularly focusing on both supervised and self-supervised methods, as well as the impact of fine-tuning on the source domain. Our analysis also highlights gaps in existing benchmark practices, guiding SF-UDA research towards more effective and general approaches. It emphasizes the importance of backbone architecture and pre-training dataset selection on SF-UDA performance, serving as an essential reference and providing key insights. Lastly, we release the source code of our experimental framework. This facilitates the construction, training, and testing of SF-UDA methods, enabling systematic large-scale experimental analysis and supporting further research efforts in this field.

==> Experiments.tex <==
In this section, we report on the carried out extended experimental analysis. 


\subsection{(SFDA Benchmarking and?) Robustness analysis}
\label{subsec:benchmark}
\textcolor{red}{
\begin{itemize}
    \item mini-intro
    \item Goal
    \item 5 methods list; Recall Motivation of methods choice
    \item Results:
        \begin{itemize}
            \item Reproducibility of the methods (same/standard datasets, same batch size, R50)
                \begin{itemize}
                    \item more seeds (average perf a bit lower than reported)
                    \item different implementations (CUDA version, etc.)
                \end{itemize}
            \item  Test robustness to different datasets (non standard datasets) (robustness to different hyper-params)
            \item  Test robustness with bigger architectures (ViT-L)
            \item  Test with different split of batch sizes and with parallelization. 
            \item SF-UDA algorithms competitive with UDA ones
            \item  Analysis of the computational time (?)
        \end{itemize}
    \item Overall Results Discussion
        \begin{itemize}
            \item Our analysis will continue with SCA and SHOT because...
                \begin{itemize}
                    \item No or few hyperparameters, much more robust, no clear model selection policy for other methods 
                    \item SCA faster, suitable for many backbones and ds
                    \item SHOT is the basis of many methods, incl. PCSR. SHOT among first SFUDA papers.
                    \item PCSR based on SHOT and adds complexity without adding much. Also a bit more costly.
                    \item ADD and NRC not robust nor stable
                \end{itemize}
        \end{itemize}
\end{itemize}}


\subsection{Analysis of the impact of pre-training}
\label{subsec:pretraining}
\textcolor{red}{
\begin{itemize}
    \item mini-intro
    \item Goal
    \item 2 baseline SFUDA methods selection, recall selection rationale (section should be self-contained)
    \item Results:
        \begin{itemize}
            \item Impact of Imagenet top-1 accuracy and Pr-training dataset for the chosen SF-UDA methods + multilinear model (**Notes:** with less emphasis than in the current paper and using Gen and DGen only as a side note to verofy quality of the features)
            \item  Standard pre-training VS semantic pre-training (from **App F**)
            \item Supervised VS Self-supervised pre-training (from **App J**)
            \item  Does size of the model count?  (not so much importance)
            \item  Normalization: Describe BN vs LN alone in the pre-training section since if we do not fine-tune the network, what we have is the pre-trained network
        \end{itemize}
    \item Overall Results Discussion

\end{itemize}}

\subsection{Analysis of the impact of the fine-tuning}
\label{subsec:finetuning}
\textcolor{red}{
\begin{itemize}
    \item mini-intro
    \item Goal
    \item 2 baseline SFUDA methods
    \item Results:
        \begin{itemize}
            \item   SHOT and SCA can still have reasonably good performance even with no fine-tuning on the source domain
            \item   SHOT VS SCA: SCA slightly worse than SHOT but 50/60 times faster (**Notes:** give less emphasis)
            \item   Normalization and Fine-tuning:
                \begin{itemize}
                \item   Fine-tuning models with BN on the source, degrades performance on the target (more in **App I**)
                \item   Failure rates for SF-UDA (modify table removing all except column BN vs LN and all the rest in appendix if possible)
                    \begin{itemize}
                    \item Discussion on the entity of the degradation
                    \end{itemize}
                \item   Experiment on one dataset
                    \begin{itemize}
                    \item   BN leads to performance drop
                    \item   ADABN can be used to recover from it
                    \item   SCA more affected than SHOT
                    \end{itemize}
                \item   Fine-tuning study grouping models by normalization layers and pre-training dataset
                \item Evaluation of performance degradation (from **App. G**)
                \end{itemize}
        \end{itemize}
    \item Overall Results Discussion
\end{itemize}}

==> R_table.tex <==
\begin{table}[t]
\caption{Comparison of adjusted $\bar{R}^2$ values between linear (considering top-1 accuracy only) and multi-linear models (with both top-1 accuracy and pre-training). Results are shown for the upper bounds (LP-IDG and FT-IDG), the lower bounds (LP-ODG and FT-ODG) and for the considered SF-UDA methods, SCA and SHOT, with and without fine-tuning (FT).}

\label{table_R}

\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lccccc}
\textbf{Method} & \textbf{}&


& \textbf{LP-IDG} & \textbf{LP-ODG} & \textbf{SCA} & \textbf{SHOT}\\
\midrule
\textbf{Linear} & 0.736 & 0.810 & 0.731 & 0.792\\
\textbf{Multi-Linear} & 0.851 & 0.935 & 0.902 & 0.890\\

 & \textbf{FT-IDG} & \textbf{FT-ODG} & \textbf{FT-SCA} & \textbf{FT-SHOT}\\
\midrule
\textbf{Linear}  & 0.803 & 0.698 & 0.668 & 0.838\\
\textbf{Multi-Linear} & 0.878 & 0.822 & 0.792 & 0.932\\
\bottomrule
\end{tabular}

%\vspace{-0.4cm}
\end{table}
